Cross-modal and Cross-domain Knowledge Transfer for Label-free 3D Segmentation

Current state-of-the-art point cloud-based perception methods usually rely on large-scale labeled data, which requires expensive manual annotations. A natural option is to explore the unsupervised methodology for 3D perception tasks. However, such methods often face substantial performance-drop difficulties. Fortunately, we found that there exist amounts of image-based datasets and an alternative can be proposed, i.e., transferring the knowledge in the 2D images to 3D point clouds. Specifically, we propose a novel approach for the challenging cross-modal and cross-domain adaptation task by fully exploring the relationship between images and point clouds and designing effective feature alignment strategies. Without any 3D labels, our method achieves state-of-the-art performance for 3D point cloud semantic segmentation on SemanticKITTI by using the knowledge of KITTI360 and GTA5, compared to existing unsupervised and weakly-supervised baselines.

==> ref.tex <==
%Entries
@inproceedings{vu2019advent,
  title={Advent: Adversarial entropy minimization for domain adaptation in semantic segmentation},
  author={Vu, Tuan-Hung and others},
  booktitle={CVPR},
  pages={2517--2526},
  year={2019}
}


@inproceedings{wang2021domain,
  title={Domain adaptive semantic segmentation with self-supervised depth estimation},
  author={Wang, Qin and others},
  booktitle={ICCV},
  pages={8515--8525},
  year={2021}
}

@inproceedings{tranheden2021dacs,
  title={Dacs: Domain adaptation via cross-domain mixed sampling},
  author={Tranheden, Wilhelm and others},
  booktitle={WACV},
  pages={1379--1389},
  year={2021}
}

@inproceedings{li2020content,
  title={Content-consistent matching for domain adaptive semantic segmentation},
  author={Li, Guangrui and others},
  booktitle={ECCV},
  pages={440--456},
  year={2020},
  organization={Springer}
}

@inproceedings{paul2020domain,
  title={Domain adaptive semantic segmentation using weak labels},
  author={Paul, Sujoy and others},
  booktitle={European conference on computer vision},
  pages={571--587},
  year={2020},
  organization={Springer}
}

@inproceedings{sautier2022image,
  title={Image-to-lidar self-supervised distillation for autonomous driving data},
  author={Sautier, Corentin and others},
  booktitle={CVPR},
  pages={9891--9901},
  year={2022}
}

@inproceedings{jaritz2020xmuda,
  title={xmuda: Cross-modal unsupervised domain adaptation for 3d semantic segmentation},
  author={Jaritz, Maximilian and others},
  booktitle={CVPR},
  pages={12605--12614},
  year={2020}
}

@inproceedings{huang2022category,
  title={Category contrast for unsupervised domain adaptation in visual tasks},
  author={Huang, Jiaxing and others},
  booktitle={CVPR},
  pages={1203--1214},
  year={2022}
}


@InProceedings{Richter_2016_ECCV,
author = {Stephan R. Richter and others},
title = {Playing for Data: {G}round Truth from Computer Games},
booktitle = {ECCV},
year = {2016},
series = {LNCS}, 
volume = {9906}, 
publisher = {Springer},
pages = {102--118}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and others},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{bottou2010large,
  title={Large-scale machine learning with stochastic gradient descent},
  author={Bottou, L{\'e}on},
  booktitle={COMPSTAT},
  pages={177--186},
  year={2010},
  organization={Springer}
}

@article{liao2022kitti,
  title={KITTI-360: A novel dataset and benchmarks for urban scene understanding in 2d and 3d},
  author={Liao, Yiyi and others},
  journal={TPAMI},
  year={2022},
  publisher={IEEE}
}

@inproceedings{wu2021dannet,
  title={Dannet: A one-stage domain adaptation network for unsupervised nighttime semantic segmentation},
  author={Wu, Xinyi and others},
  booktitle={CVPR},
  pages={15769--15778},
  year={2021}
}

% ================

@inproceedings{behley2019semantickitti,
  title={Semantickitti: A dataset for semantic scene understanding of lidar sequences},
  author={Behley, Jens and others},
  booktitle={ICCV},
  pages={9297--9307},
  year={2019}
}


@inproceedings{zhu2021cylindrical,
  title={Cylindrical and asymmetrical 3D convolution networks for lidar segmentation},
  author={Zhu, Xinge and others},
  booktitle={CVPR},
  pages={9939--9948},
  year={2021}
}

@article{goodfellow2020generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian and others},
  journal={CACM},
  volume={63},
  number={11},
  pages={139--144},
  year={2020},
  publisher={ACM New York, NY, USA}
}

% ================
@inproceedings{guo2022simt,
  title={Simt: handling open-set noise for domain adaptive semantic segmentation},
  author={Guo, Xiaoqing and others},
  booktitle={CVPR},
  pages={7032--7041},
  year={2022}
}

@inproceedings{zhang2021prototypical,
  title={Prototypical pseudo label denoising and target structure learning for domain adaptive semantic segmentation},
  author={Zhang, Pan and others},
  booktitle={CVPR},
  pages={12414--12424},
  year={2021}
}

@inproceedings{liu2022less,
  title={Less: Label-efficient semantic segmentation for lidar point clouds},
  author={Liu, Minghua and others},
  booktitle={ECCV},
  pages={70--89},
  year={2022},
  organization={Springer}
}

@inproceedings{unal2022scribble,
  title={Scribble-supervised lidar semantic segmentation},
  author={Unal, Ozan and others},
  booktitle={CVPR},
  pages={2697--2707},
  year={2022}
}

@inproceedings{shi2022weakly,
  title={Weakly supervised segmentation on outdoor 4d point clouds with temporal matching and spatial graph propagation},
  author={Shi, Hanyu and others},
  booktitle={CVPR},
  pages={11840--11849},
  year={2022}
}

@article{fischler1981random,
  title={Random sample consensus: a paradigm for model fitting with applications to image analysis and automated cartography},
  author={Fischler, Martin A and others},
  journal={CACM},
  volume={24},
  number={6},
  pages={381--395},
  year={1981},
  publisher={ACM New York, NY, USA}
}



@inproceedings{ronneberger2015u,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and others},
  booktitle={MICCAI},
  pages={234--241},
  year={2015},
  organization={Springer}
}

@inproceedings{wu2018squeezeseg,
  title={Squeezeseg: Convolutional neural nets with recurrent crf for real-time road-object segmentation from 3d lidar point cloud},
  author={Wu, Bichen and others},
  booktitle={ICRA},
  pages={1887--1893},
  year={2018},
  organization={IEEE}
}

@inproceedings{gerdzhev2021tornado,
  title={Tornado-net: multiview total variation semantic segmentation with diamond inception module},
  author={Gerdzhev, Martin and others},
  booktitle={ICRA},
  pages={9543--9549},
  year={2021},
  organization={IEEE}
}


@article{wang2019dynamic,
  title={Dynamic graph cnn for learning on point clouds},
  author={Wang, Yue and others},
  journal={TOG},
  volume={38},
  number={5},
  pages={1--12},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@article{chen2017deeplab,
  title={Deeplab: Semantic image segmentation with deep convolutional nets, atrous convolution, and fully connected crfs},
  author={Chen, Liang-Chieh and others},
  journal={TPAMI},
  volume={40},
  number={4},
  pages={834--848},
  year={2017},
  publisher={IEEE}
}

@inproceedings{bian2022unsupervised,
  title={Unsupervised Domain Adaptation for Point Cloud Semantic Segmentation via Graph Matching},
  author={Bian, Yikai and others},
  booktitle={IROS},
  pages={9899--9904},
  year={2022},
  organization={IEEE}
}

@inproceedings{li2022sigma,
  title={Sigma: Semantic-complete graph matching for domain adaptive object detection},
  author={Li, Wuyang and others},
  booktitle={CVPR},
  pages={5291--5300},
  year={2022}
}



@inproceedings{milioto2019rangenet++,
  title={Rangenet++: Fast and accurate lidar semantic segmentation},
  author={Milioto, Andres and others},
  booktitle={IROS},
  pages={4213--4220},
  year={2019},
  organization={IEEE}
}

@article{cortinhal2020salsanext,
  title={Salsanext: Fast, uncertainty-aware semantic segmentation of lidar point clouds for autonomous driving},
  author={Cortinhal, Tiago and others},
  journal={arXiv:2003.03653},
  year={2020}
}




@inproceedings{wu2019squeezesegv2,
  title={Squeezesegv2: Improved model structure and unsupervised domain adaptation for road-object segmentation from a lidar point cloud},
  author={Wu, Bichen and others},
  booktitle={ICRA},
  pages={4376--4382},
  year={2019},
  organization={IEEE}
}

@inproceedings{liu2021one,
  title={One thing one click: A self-training approach for weakly supervised 3d semantic segmentation},
  author={Liu, Zhengzhe and others},
  booktitle={CVPR},
  pages={1726--1736},
  year={2021}
}

@inproceedings{ren20213d,
  title={3d spatial recognition without spatially labeled 3d},
  author={Ren, Zhongzheng and others},
  booktitle={CVPR},
  pages={13204--13213},
  year={2021}
}

@inproceedings{hou2022point,
  title={Point-to-voxel knowledge distillation for lidar semantic segmentation},
  author={Hou, Yuenan and others},
  booktitle={CVPR},
  pages={8479--8488},
  year={2022}
}

@article{guo2020deep,
  title={Deep learning for 3d point clouds: A survey},
  author={Guo, Yulan and others},
  journal={TPAMI},
  volume={43},
  number={12},
  pages={4338--4364},
  year={2020},
  publisher={IEEE}
}

@inproceedings{zhao2021few,
  title={Few-shot 3d point cloud semantic segmentation},
  author={Zhao, Na and others},
  booktitle={CVPR},
  pages={8873--8882},
  year={2021}
}

@article{mei2019semantic,
  title={Semantic segmentation of 3d lidar data in dynamic scene using semi-supervised learning},
  author={Mei, Jilin and others},
  journal={T-ITS},
  volume={21},
  number={6},
  pages={2496--2509},
  year={2019},
  publisher={IEEE}
}


@article{peng2022cl3d,
  title={CL3D: Unsupervised Domain Adaptation for Cross-LiDAR 3D Detection},
  author={Peng, Xidong and others},
  journal={arXiv:2212.00244},
  year={2022}
}

@inproceedings{yan20222dpass,
  title={2dpass: 2d priors assisted semantic segmentation on lidar point clouds},
  author={Yan, Xu and others},
  booktitle={ECCV},
  pages={677--695},
  year={2022},
  organization={Springer}
}


@inproceedings{bogoslavskyi2016fast,
  title={Fast range image-based segmentation of sparse 3D laser scans for online operation},
  author={Bogoslavskyi, Igor and others},
  booktitle={IROS},
  pages={163--169},
  year={2016},
  organization={IEEE}
}

@inproceedings{langer2020domain,
  title={Domain transfer for semantic segmentation of LiDAR data using deep neural networks},
  author={Langer, Ferdinand and others},
  booktitle={IROS},
  pages={8263--8270},
  year={2020},
  organization={IEEE}
}

==> tables.tex <==
\begin{table}[hbt!]
\tiny
\caption{ Ours is the result of our trained model with fine-tuning. The first row presents the results of using state-of-the-art semantic segmentation backbone DeepLabV2 \cite{chen2017deeplab}. The medium five rows are 2D UDA methods \cite{vu2019advent,huang2022category,li2020content,tranheden2021dacs,wu2021dannet}. }
\begin{subtable}[H]{0.45\textwidth}
\caption{KITTI360\ \textrightarrow \ SemanticKITTI.}
\centering
  \begin{tabular}{c c c cccccc }
    % \toprule
    % \multicolumn{15}{c}{KITTI360 $\rightarrow$ SemanticKITTI}\\
    \hline
    Method & \rotatebox[origin=c]{90}{Road} & \rotatebox[origin=c]{90}{Sidewalk} & \rotatebox[origin=c]{90}{Building}  & \rotatebox[origin=c]{90}{Vegetation} & \rotatebox[origin=c]{90}{Terrain} &  \rotatebox[origin=c]{90}{Car} & mIoU \\
    \hline
    DeepLabV2 &17.96 & 6.79& 5.34& 33.24& 1.07& 0.71 &10.85 \\
    \hline
    AdvEnt & 20.34 & 10.87 & 14.48  & 34.13 & 0.06 & 0.21 & 13.35\\
    CaCo & 27.43 & 8.73 & 18.05  & 34.65 & 6.15 & 0.43 & 15.91 \\
    CCM & 0.01 & 5.63 & \textbf{24.15}   & 20.83 & 0 & 7.11  & 9.62 \\
    DACS & 19.35 & 7.44 & 0 & 0.13 & 0 & 6.64 & 5.59 \\
    DANNet & 15.30 & 0 & 13.75  & 31.46 & 0 & 0 & 10.09 \\
    % corda &&&&&&&&&&&&&& \\
    \hline
    %Ours (car+DGCNN) &35.68 & 19.65& 1.66& 0.22& 0.08& 0& 46.40& 6.27& 0& 23.22& 0& 0& 0& 10.24/19.01 \\
    %Ours & 45.05 & 21.50 & 2.18 & 0.02 & 45.99 & 4.18  & 28.49 & 21.06\\
    %Ours & 33.89 & 18.40 & 11.84 & 0.29 & 34.69 & 7.52 & 28.84 & 19.35 \\
    %1w-6000
    Ours  & \textbf{45.05} & \textbf{21.50} & 2.18 & \textbf{45.99} & \textbf{4.18}  & \textbf{28.49} & \textbf{24.57} \\
    \hline
\end{tabular}
\label{tab:360sem}
\end{subtable}
\hfill
% \hspace{-10ex}  
 \begin{subtable}[ht]{0.475\textwidth}
 \caption{GTA5\ \textrightarrow  \ SemanticKITTI.}
\centering
  \begin{tabular}{c c c cccccc}
    % \toprule
    % \multicolumn{15}{c}{GTA5 $\rightarrow$ SemanticKITTI}\\
    % \midrule
    \hline    
    Method & \rotatebox[origin=c]{90}{Road} & \rotatebox[origin=c]{90}{Sidewalk} & \rotatebox[origin=c]{90}{Building} & \rotatebox[origin=c]{90}{Vegetation} & \rotatebox[origin=c]{90}{Terrain} &  \rotatebox[origin=c]{90}{Car} & mIoU \\
    \hline
    %DeepLabV2 & 25.63 & 6.07 & 0.56 & \textbf{35.94} & 1.92 & 0.13 & 11.71\\
    DeepLabV2 & 18.87 & 0 & 24.19 & 17.46 & 0 & 0.97 & 10.24 \\
    \hline
    AdvEnt & 0.65 & 0 & 11.96  & 12.32 & 0 & 1.45 & 4.40 \\
    CaCo & 12.06 & 13.85 &  17.21  & 21.69 & 3.14 & 2.61 & 11.76 \\
    CCM & 0 & 2.18 & 20.47  & 20.14 & 0.27 & 0.83 & 7.32 \\
    DACS & 23.73 & 0 & 17.02   & 0 & 0 & 0 & 6.79 \\
    DANNet & 1.67 & \textbf{18.28} & \textbf{28.19} & 0 & \textbf{12.17} & 0 & 10.05 \\
    % corda & 21.82 & 12.01 & 12.09 & 0.06 & 0.77 & 0 & 17.04 & 0.27 & 0 & 0 & 0 & 0 & 0 & 4.93 \\
    \hline
    %Ours &30.38 & 20.67 & 19.28 & 0 & 10.71 & 8.93 & 0.14 & 12.87 \\
    Ours & \textbf{37.63} & 1.23 & 27.79 & \textbf{31.40} & 0.03 & \textbf{30.00} & \textbf{21.35} \\
  \hline
\end{tabular}
\vspace{-0.5ex}  
\label{tab:gta5sem}
\end{subtable}
\vspace{-1.25ex}     
\label{tab:main table}
\end{table}



